Laugh at Your Own Pace: Basic Performance Evaluation of Language Learning Assistance by Adjustment of Video Playback Speeds Based on Laughter Detection

Among various methods to learn a second language (L2), such as listening and shadowing, Extensive Viewing involves learning L2 by watching many videos. However, it is difficult for many L2 learners to smoothly and effortlessly comprehend video contents made for native speakers at the original speed. Therefore, we developed a language learning assistance system that automatically adjusts the playback speed according to the learner's comprehension. Our system judges that learners understand the contents if they laugh at the punchlines of comedy dramas, and vice versa. Experimental results show that this system supports learners with relatively low L2 ability (under 700 in TOEIC Score in the experimental condition) to understand video contents. Our system can widen learners' possible options of native speakers' videos as Extensive Viewing material.

==> tex/03_preli_study.tex <==
We conducted a preliminary experiment to examine whether learners behave differently depending on their comprehension towards video contents during Extensive Viewing.
5 participant joined this experiment. 
We selected English as a target language.
We told the participants that they join this experiment with their ordinary eyewear conditions and make their face easy to see such as brushing up bangs during the experiment.

